Secret Key Generation from Sparse Wireless Channels: Ergodic Capacity and Secrecy Outage

This paper investigates generation of a secret key from a reciprocal wireless channel. In particular we consider wireless channels that exhibit sparse structure in the wideband regime and the impact of the sparsity on the secret key capacity. We explore this problem in two steps. First, we study key generation from a state-dependent discrete memoryless multiple source. The state of source captures the effect of channel sparsity. Secondly, we consider a wireless channel model that captures channel sparsity and correlation between the legitimate users' channel and the eavesdropper's channel. Such dependency can significantly reduce the secret key capacity. According to system delay requirements, two performance measures are considered: (i) ergodic secret key capacity and (ii) outage probability. We show that in the wideband regime when a white sounding sequence is adopted, a sparser channel can achieve a higher ergodic secret key rate than a richer channel can. For outage performance, we show that if the users generate secret keys at a fraction of the ergodic capacity, the outage probability will decay exponentially in signal bandwidth. Moreover, a larger exponent is achieved by a richer channel.

==> Proof_mutual_info.tex <==

Since from the model in \eqref{equ:sparse_channel_output}, $\bx-\bh-\by$ forms a Markov chain. By the same reason in \eqref{equ:gedms.Iab_muinfo_intersect},
\begin{align}
  I(\bx;\by) &= I(\bx;\bh) + I(\by;\bh) - I(\bx,\by; \bh) \nnum \\
             &= I(\bS^H \bx;\bh) + I(\bS^H\by;\bh) - I(\bS^H\bx,\bS^H\by; \bh) \label{equ:three_sum_Ixy}\ .
\end{align}
The last equality is due to the fact that $\bS^H \bx$ and $\bS^H \by$ are sufficient statistics of $\bx$ and $\by$, respectively. Each term in \eqref{equ:three_sum_Ixy} can be calculated using  the fact that $\bS^H \bx$, $\bS^H \by$ and $\bh$ form parallel channels and each component channel is according to \eqref{equ:scalar_xy}-\eqref{equ:eve_equiv_rx} and. We get
%
\begin{align*}
  I(\bx;\by) = \sum_{\ell=1}^L \log(1 + \nu^2_\ell \snr_a ) + \log(1 + \nu^2_\ell \snr_b ) - \log(1 + \nu^2_\ell (\snr_a+ \snr_b) ) = \sum_{\ell=1}^L \Iab(\nu^2_\ell \snr_a, \nu^2_\ell \snr_b) \ .
\end{align*}
Similarly, 
%
\begin{align*}
  I(\bx;\bz) &= \sum_{\ell=1}^L \log(1 + \nu^2_\ell \snr_a ) 
            + \log\left( 1 + \frac{q_\ell \nu^2_\ell |\eta|^2 \snr_e}{\nu^2_\ell (1-|\eta|^2) \snr_e + 1} \right)
            - \log\left(1 + \nu^2_\ell \snr_a  + \frac{q_\ell \nu^2_\ell |\eta|^2 \snr_e}{\nu^2_\ell (1-|\eta|^2) \snr_e + 1} \right)  \\
            &= \sum_{\ell=1}^L q_\ell \Iae(\nu^2_\ell \snr_a, \nu^2_\ell \snr_b) \ .
\end{align*}
where $\Iae(\cdot)$ is defined in \eqref{equ:eve_Iae}. 



==> chapter_main.tex <==

\chapter{Sparse Channel and Correlated Eavesdropping in the Wideband Regime}\label{ch:sparse}   % level 1

\graphicspath{{./ch5/figures/}}

\input{ch5/introduction}

\input{ch5/system_model3}

\input{ch5/ergodic}

\input{ch5/outage}

\input{ch5/conclusion}

\input{ch5/appendix}




==> ergodic.tex <==
\section{Lower Bound of Ergodic Secret Key Capacity}
\label{sec:sparse.ergodic}

When the code block $n$ is sufficient large such that the ergodic behavior of $Q_\ell$ can be observed in a code block. The secret key capacity in the Shannon's sense is well defined and we call it the \emph{ergodic secret key capacity}. The theorems developed in [?] \textbf{(thc: ChouEtal'10)} are applied in this case.

We are interested in the ergodic secret key capacity in the wideband regime and would like to know how the sparsity parameter $\delta$ influences the capacity. Note that it is unlike the rich scattering environment discussed in [?] \textbf{(thc: add reference)} where eavesdropper's observation is useless for estimating the key.
We need to characterize the degradedness condition to guarantee the positivity of the secret key rate.


\subsection*{\normalsize Mutual information}


We first look the expressions of mutual information $I(\bx;\by|\bs)$ and  $I(\bx;\bz|\bs)$ of the vector channels \eqref{equ:sparse_channel_output} and \eqref{equ:sparse_Eve_output}.

\begin{prop}[Mutual information of vector source]\label{prop:mutual_info}
    Let $\bQ = [Q_1,\cdots,Q_L]$,  then
    \begin{subequations} \label{equ:vector_muInfo}
    \begin{align}
      I(\bx;\by|\bs) &\doteq \sum_{\ell=1}^L \Iab(\varh_\ell \snr_a, \varh_\ell \snr_b) \label{equ:Ixy_givenS}\\
      I(\bx;\bz|\bs) &\doteq \sum_{\ell=1}^L Q_\ell \Iae(\varh_\ell \snr_a, \varh_\ell \snr_e) \label{equ:Ixz_givenS}
    \end{align}
    \end{subequations}
    where
    \begin{align}
        &\Iab(\snr_a,\snr_b) = \log \left( \frac{ (1+\snr_a)(1+\snr_b) }{1+ \snr_a + \snr_b} \right) \ , \\
        &\Iae(\snr_a, \snr_e) = \log \left( \frac{ (1+\snr_a)(1+\snr_e) }{1+ \snr_a \snr_e (1-|\eta|^2) +\snr_a + \snr_e} \right) \ . \label{equ:eve_Iae}
    \end{align}
    $\snr_a = \frac{P}{\nvar_a}$, $\snr_b = \frac{P}{\nvar_b}$ and $\snr_e = \frac{P}{\nvar_e}$.
\end{prop}

The detailed derivation is presented in Section \ref{sec:sparse.Proof_mutual_info}. Equation \eqref{equ:vector_muInfo} says the mutual information of the vector variables can be written as a sum of the mutual information in each channel dimension. Eve's information $I(\bx;\bz|\bs)$ is masked by $\bQ$ due to  a partial overlap between $\bh$ and $\tilbh$.
From \eqref{equ:eve_Iae}, a small correlation coefficient $|\eta|^2$ results in a small Eve's information. $I(\bx;\bz|\bs) \to 0$ as $|\eta|^2 \to 0$.


% ==== degraded =====
\subsection*{\normalsize  Degradedness}

Because the Eve's channel is correlated to the main channel, she may get a good estimation of $\bh$ if she has a higher SNR than the users.
To guarantee the positivity of the secret key rate, we need to characterize the condition that eavesdropper has a worse observations than the users. To see this, we first look the subspace where $q_\ell=1$. Projecting the channel outputs onto the space $\bs_\ell$,
\begin{subequations} \label{equ:scalar_xy}
\begin{align}
   x_\ell &= \bs_\ell^H \bx \doteq P h_\ell + w_{1,\ell} \\
   y_\ell &= \bs_\ell^H \by \doteq P h_\ell + w_{2,\ell} \ .
\end{align}
\end{subequations}
Because the sounding signal is a (asymptotic) white sequence, $x_\ell$ (and $y_\ell$) are sufficient statistic for estimating $h_\ell$. The noise $w_{1,\ell}$ (resp. $w_{2,\ell}$) is a zero mean complex Gaussian with variance $P\nvar_a$ (resp. $P\nvar_b$).
Similarly, Eve's sufficient static is
\begin{equation}\label{equ:eve_equiv_rx}
   z_\ell = \bs_\ell^H \bz \doteq P \tilh_\ell + w_{3,\ell} \equiv P \eta h_\ell +
            P \sqrt{1 - |\eta|^2} h'_\ell + w_{3,\ell} \ .
\end{equation}
Because of $\rho(h_\ell, \tilh_\ell) = \eta$, we can equivalently write $\tilh_\ell$ in two parts as it is done in the above. One is statistically aligned with $h_\ell$ and the other $h'_\ell$ has the same distribution but independent of $h_\ell$.
We see from \eqref{equ:eve_equiv_rx} that Eve's observation $z_\ell$ contains two types of noise: one is the receiving noise $w_{3,\ell}$ and the other is due to the uncorrelated $h'_\ell$. The $z_\ell$ is a degraded version of $y_\ell$ if she has a smaller SNR than Bob, that is
\begin{equation}
    \frac{ \varh_\ell P }{\nvar_b} > \frac{|\eta|^2 \varh_\ell P}{(1-|\eta|^2)\varh_\ell P + \nvar_e}  \ .
\end{equation}
Otherwise, $y_\ell$ is a degraded version of $z_\ell$. We can see that if the sounding signal power is small, in particular, $(1-|\eta|^2) \varh_\ell P < |\eta|^2 \nvar_b - \nvar_e$, Bob's output is noisier and no positive key rate can be extracted in this subspace. This is because when $P$ is small, one of Eve's noise (due to $h'_\ell$) is decreased.
It is observed in \cite{chou_isit10} that there is a cutoff SNR below which the secret key capacity is zero.

If all the users (Alice, Bob and Eve) are with the same SNR, \ie, $\nvar_a=\nvar_b=\nvar_e = \nvar$, the secret key capacity is always positive because Eve has an extra noise (due to $h'_\ell$). In the following, we focus on the equal-SNR case and see how the system parameters (\eg, $W$ and $P$) affect the capacity in the wideband regime.

% ==============================================================
\subsection*{\normalsize Ergodic secret key capacity lower bound in the wideband regime}


The instantaneous and ergodic secret key rates for the equal-SNR case are
%
\begin{align}
    \Iinst(\snr, W|\bQ) &= I(\bx;\by|\bs) - I(\bx;\bz|\bs) \nnum \\
        &= \sum_{\ell=1}^L \Iab(\varh_\ell \snr) - Q_\ell \Iae(\varh_\ell \snr) \label{equ:Iinst_defn}\\
    \Ierg(\snr, W) &= \rvE[\Iinst(\snr, W|\bQ)] \nnum \\
        &= \sum_{\ell=1}^L \Iab(\varh_\ell \snr) - \theta \Iae(\varh_\ell \snr) \label{equ:Ierg_defn}
\end{align}
%
where $\snr \triangleq \frac{P}{\nvar}$ and the expectation is over the random vector $\bQ$. $\Iab(\snr)$ (resp. $\Iae(\snr)$) is a shorthand for $\Iab(\snr, \snr)$ (resp. $\Iae(\snr, \snr)$).

The ergodic secret key capacity in the wideband regime with power constraint $P$ is lower bounded by
\begin{equation}\label{equ:ergodic_skcap_LU}
    \Cerg(P,W) \geq \CergLB(P,W) \triangleq \max_{\bs:\rvE[\bs^H\bs]\leq P} \Ierg(\snr, W)
\end{equation}
%
\begin{remark}
Note that we say the right hand side of \eqref{equ:ergodic_skcap_LU} a lower bound because the achievable ergodic key rate \eqref{equ:Ierg_defn} is obtained by assuming $\bs$ is a white sequence (\cf \eqref{equ:white_sequence_assumption}). It remains open if there exists a non-white sequence (subject to an average power constraint) which can achieve a higher ergodic key rate.
\end{remark}

When $W$ increases, $L$ increases sub-linearly according to \eqref{equ:sublinear_law} and $\varh_\ell$ gets smaller. In order to see the clear behavior in terms of $W$ and $\snr$, we look a uniform power delay profile $\varh_\ell = \frac{1}{L}$ and use the following approximations for $x \ll 1$
\begin{subequations}\label{equ:lowSNR_muInfo_approx}
\begin{align}
    &\Iab(\snr) \approx \frac{x^2}{\ln 2}  \ , \\
    &\Iae(\snr) \approx \frac{|\eta|^2 x^2}{\ln 2}  \ .
\end{align}
\end{subequations}
We get ergodic secret key rate in the wideband regime
\begin{equation}\label{equ:Ierg_wideband_approx}
    \Ierg(\snr, W) \thickapprox \frac{1-\theta |\eta|^2}{\ln 2} \frac{\snr^2}{(\taum W)^{\delta}} \ .
\end{equation}

\iffalse
Using approximations for $\Iab(\snr)$ and $\Iae(\snr)$ for ,
\begin{align}
  \text{In high SNR:}  &\quad \Iab(\snr) \approx \log\left(1+ \frac{\snr}{2} \right)
        \quad \text{and} \quad  \Iab(\snr) \approx \log\left(\frac{1}{1-|\eta|^2} \right) \\
  \text{In low SNR:}  &\quad \Iab(\snr) \approx \snr^2
        \quad \text{and} \quad  \Iab(\snr) \approx |\eta|^2 \snr^2 \ ,
\end{align}
and applying $\varh_\ell = \frac{1}{L}$ if the true power delay profile is unknown. We get ergodic secret key capacity approximations in high and low SNR regimes:
\fi

If $W$ is fixed (but large), we see $\Ierg \propto \snr^2$. This is the same behavior of the low SNR regime as we studied in Chapter \ref{ch:gaussian_edms} because the \emph{sounding power} is spread out in a wide bandwidth.
From the same reason in Theorem \ref{thm:Gaussian_sk_capacity}, we can increase the peakyness in \emph{time domain} by using an on-off signal to get a higher the key rate. In particular,
\begin{equation}\label{equ:ergodic_skcap}
    \CergLB(P, W) = \max_{0<\tsf \le 1} \lambda \Ierg \left(\frac{\snr}{\tsf}, W \right) \ .
\end{equation}
On the other hand, $\Ierg(\snr, W)$ in \eqref{equ:Ierg_wideband_approx} becomes smaller for a larger $\delta$. This means that for a fixed $W$, a richer channel spread out the \emph{channel power} to a large DoF. Furthermore, since the way to change channel DoF is through bandwidth $W$ (see \eqref{equ:sublinear_law}), this implies the way to achieve $\CergLB(P, W)$ is to find an appropriate signal dimension in either \emph{time} or \emph{frequency} domain.


Figure \ref{fig:Ierg_vs_snr} shows $\Ierg(\snr, W)$ versus $\snr$ fixing $W=10$MHz and values $\delta \in [0.5, 1]$. We see that a sparser channel (small $\delta$) achieves a higher key rate at a low SNR because it concentrates all channel power on a few DoF. A richer channel (large $\delta$) gets a higher key rate at a high SNR since this is DoF-limited regime.
%
\begin{figure}
  \centering
  \includegraphics[width=0.45\textwidth]{Ierg_vs_snr.eps}\\
  \caption{$\Ierg(\snr,W)$ vs. $\snr$. $W$ is fixed to 10MHz, $\taum =$ 100ns, $\theta=0.5$ and $\eta=0.1$. Sparsity parameter $0.5 \leq \delta \leq 1$.}
  \label{fig:Ierg_vs_snr}
\end{figure}
%
Figure \ref{fig:Ierg_vs_w} shows $\Ierg(\snr, W)$ versus $W$. In Figure \ref{fig:Ierg_vs_w.1}, $\snr$ is fixed to $10$dB and different values of sparsity $\delta$ in $[0.5,1]$ are plotted. This shows the wideband (low-SNR) regime, a large $\delta$ gets a small key rate.  In Figure \ref{fig:Ierg_vs_w.2}, $\delta=0.8$ is fixed and $\snr$ varies from 10dB to 30dB. We can see for each SNR, there is one $W^*$ achieves the highest key rate.
%
\begin{figure}
  \centering
  \subfigure[]
  {\includegraphics[width=0.45\textwidth]{Ierg_vs_w-1.eps}       \label{fig:Ierg_vs_w.1} }
  \subfigure[]
  {\includegraphics[width=0.45\textwidth]{Ierg_vs_w-2.eps}       \label{fig:Ierg_vs_w.2} }
  \caption{$\Ierg(\snr,W)$ vs. $W$
      \subref{fig:Ierg_vs_w.1} $0.5 \leq \delta \leq 1$, $\snr=10$ dB.
      \subref{fig:Ierg_vs_w.2} $10$dB $\leq \snr \leq 30$dB, $\delta=0.8$.}
  \label{fig:Ierg_vs_w}
\end{figure}








==> outage.tex <==
\section{Secrecy Outage}
\label{sec:sparse.outage}

When the application has a stringent delay requirement, the code block length is small such that a state of overlapping pattern $\bQ$ cannot be revisited within the code block. The users might suffer from a significant key information leakage due to a worse state of $\bQ$. In particular, satisfying the secrecy condition \eqref{equ:secrecy_condition} can be problematic.
The secret key capacity in Shannon's sense is not well-defined in this case. One of a natural information-theoretic performance measure is based on the key rate versus secrecy outage probability characteristics, where the later is defined as the probability of event that the considered key generation rate cannot be supported by the instantaneous channel using the best on-off sounding scheme. More precisely,
%
when $\bQ = [Q_1, \cdots, Q_L]$ is fixed, we consider a \emph{secrecy outage} has happened if
\begin{equation}
    \keyrate > \tsfOpt\Iinst\left(\frac{\snr}{\tsfOpt}, W \big|\bQ \right) \ .
\end{equation}
where $\tsfOpt$ is the optimal time-sharing parameter which achieves the ergodic secret key rate in \eqref{equ:ergodic_skcap}.

\subsection*{\normalsize Information Leakage}

Because two conditions are required by the system: reliability condition \eqref{equ:reliable_condition_edms} and secrecy condition  \eqref{equ:secrecy_condition_edms}, it is important to clarify which one fails if the secrecy outage event occurs and what leaks to Eve.
%
In the following lemma we show that if Alice and Bob can reliably agree with the same key, the secrecy outage event implies that there is a non-negligible portion of the key information leaking to Eve.

\begin{lemma}[Information leakage]\label{lemma:info_leakage}
    Fix a $\bQ$, if Alice and Bob can reliably agree with a key (\ie, $\Pr[\keyA \neq \keyB] < \epsilon $) with a rate $\keyrate$ such that $\keyrate - \Iinst(\snr, W|\bq) = \triangle R > 0$, then
    \begin{equation}
        I(\keyA ; \srcEn, \Phi) \ge n (\triangle R - 2 \epsilon) \ .
    \end{equation}
\end{lemma}
%
The proof is given in Section \ref{sec:sparse.Proof_info_leakage}.



\subsection*{\normalsize Secrecy outage probability}

The \emph{secrecy outage probability} (or simply \emph{outage probability}) is the probability of the secrecy outage event, \ie,
\begin{equation} \label{equ:outage_prob_defn}
    \Pout(R) = \Pr\left(R \geq \tsfOpt\Iinst\left(\frac{\snr}{\tsfOpt}, W \big|\bQ \right) \right) \ .
\end{equation}
%
The value of $\Pout(R)$ is served as a security index which measures how secure the key would be in a probabilistic sense for the given model.
%
We are interested in how $\Pout(R)$ decreases when the considered key rate is reduced. In particular, we want to upper bound  $\Pout(R)$ when $R = \alpha \CergLB(P,W)$, $0 < \alpha\leq 1$.
We again assume a uniform power delay profile $\varh_\ell = \frac{1}{L}$  and define $J = \sum_{\ell=1}^L Q_\ell$. Combine \eqref{equ:outage_prob_defn}, \eqref{equ:ergodic_skcap}, \eqref{equ:Iinst_defn} and \eqref{equ:Ierg_defn}, the outage probability can be rearranged as
%
\begin{align}
    &\Pout(\alpha \Cerg(P,W)) = \Pr\left( J \geq L a \right) \label{equ:outage_rearranged}\\
    \text{where} \quad
    & a= (1-\alpha)A + \alpha \theta \\
    \text{and} \quad
    & A = \frac{\Iab\left( \frac{1}{L}\frac{\snr}{\tsfOpt} \right)}{\Iae\left( \frac{1}{L}\frac{\snr}{\tsfOpt}\right)} \ .
\end{align}

Note that random variable $J$ is binomial $\randBino{L}{\theta}$ distributed. When the correlation coefficient $|\eta|^2$ is strictly less than one, $\Iab(x)>\Iae(x)$ from their definitions in \eqref{equ:gaussain_SK_rate} and \eqref{equ:eve_Iae}. When this case happens, $A>1$ and thus $a > \theta$. The outage event \eqref{equ:outage_rearranged} is a rare event and has a probability exponentially small as $L$ (the channel DoF) getting large. We then use large deviation theory \cite{Arratia89, CoverIT} to upper bound the tail probability of binomial distribution.
\begin{lemma}[Theorem 1 in \cite{Arratia89}]
   Let $S_n$ be a binomial random variable $\randBino{n}{p}$. For $p< a <1$, and for $n=1,2,3,\cdots$,
   \begin{equation}
      \Pr(S_n \geq a n) \leq 2^{-n D(a\|p)}
   \end{equation}
   where
   \begin{equation}
      D(a\|p) \equiv a \log \frac{a}{p} + (1-a)\log \frac{(1-a)}{1-p}
   \end{equation}
   is the Kullback-Leibler divergence between the probability distributions $\randBern{a}$ and $\randBern{p}$.
\end{lemma}
In \cite{Arratia89}, the authors show this upper bound is tighter than the tail probability by Gaussian approximation.

By this lemma, the outage probability is upper bounded as
%
\begin{equation} \label{equ:outage_UB}
    \Pout(\alpha \Cerg(P,W)) \leq 2^{-L D(a\|\theta)} \ .
\end{equation}
%
Note that from \eqref{equ:outage_rearranged}-\eqref{equ:outage_UB}, the SNR (or equivalently, power $P$) only affects the mutual information ratio $A$. The bandwidth $W$  influences the outage probability in a more complicated way.
We see that the exponent in \eqref{equ:outage_UB} consists of two terms: $L$ and $D(a\|\theta)$. Roughly speaking,  the first term $L$ considers the channel DoF upon which the correlated sources are obtained; the second term $D(a\|\theta)$ considers the power allocated in each DoF via the mutual information ratio $A$.
As we see in the ergodic case, there is a tradeoff between these two factors, resulting in an optimal designed bandwidth $W^*$. To see the effect in outage performance, we look the wideband regime in the following.


% ==========================================================

\subsection*{\normalsize Wideband regime}

When $W$ is large, each subspace is in the low-SNR regime. Use approximations \eqref{equ:lowSNR_muInfo_approx}, we can approximate $A \approx \frac{1}{|\eta|^2}$, and $a$ is approximately a constant (not function of $\snr$).
The exponent is proportional to $W^\delta$ and is not a function of SNR.
Figure \ref{fig:outageExp_vs_w} shows the numerical results of the secrecy outage exponent $L D(a\|\theta)$ in the wideband regime.
We see that (i) for $\delta<1$ the curve is sub-linear in $W$ (the curve with $\delta=1$ is close to linear in $W$) and (ii) a richer channel (larger $\delta$) has a larger exponent. The later one shows that the channel sparsity has different impacts on the ergodic performance and the outage performance. This can be understood by noting that a larger channel DoF drives the condition toward the ergodic regime faster in which the secrecy condition \eqref{equ:secrecy_condition} is fulfilled.

\begin{figure}
  \centering
  \includegraphics[width=0.45\textwidth]{outageExp_vs_w.eps}\\
  \caption{Outage exponent $L D(a\|\theta)$ vs. bandwith $W$. $\taum =$ 100ns, $\theta=0.5$ and $\eta=0.1$. Sparsity parameter is between $0.5 \leq \delta \leq 1$.}
  \label{fig:outageExp_vs_w}
\end{figure} 

==> styles/defs.tex <==
% \input{../gww_defs}
% \input{../gww_chars}

\newcommand{\theterm}{Spring 1999}

\newcounter{psctr}
\newcounter{probctr}[psctr]
%\renewcommand{\theprobctr}{\arabic{psctr}.\arabic{probctr}}
\newcommand{\problem}[1]{%
\addtocounter{probctr}{1}
\vspace{.15in}

\noindent\textbf{Problem \thepsctr.\theprobctr}\nopagebreak

\noindent{#1}

}
\newcommand{\extraproblem}[1]{%
\addtocounter{probctr}{1}
\vspace{.15in}

\noindent\textbf{Problem \thepsctr.\theprobctr\ (practice)}\nopagebreak

\noindent{#1}

}

\DeclareMathAlphabet{\mathbsf}{OT1}{cmss}{bx}{n}% bold sans serif
\DeclareMathAlphabet{\mathssf}{OT1}{cmss}{m}{sl}% slanted sans serif

% define some useful uppercase Greek letters in regular and bold sf
\DeclareSymbolFont{bsfletters}{OT1}{cmss}{bx}{n}
\DeclareSymbolFont{ssfletters}{OT1}{cmss}{m}{n}
\DeclareMathSymbol{\bsfGamma}{0}{bsfletters}{'000}
\DeclareMathSymbol{\ssfGamma}{0}{ssfletters}{'000}
\DeclareMathSymbol{\bsfDelta}{0}{bsfletters}{'001}
\DeclareMathSymbol{\ssfDelta}{0}{ssfletters}{'001}
\DeclareMathSymbol{\bsfTheta}{0}{bsfletters}{'002}
\DeclareMathSymbol{\ssfTheta}{0}{ssfletters}{'002}
\DeclareMathSymbol{\bsfLambda}{0}{bsfletters}{'003}
\DeclareMathSymbol{\ssfLambda}{0}{ssfletters}{'003}
\DeclareMathSymbol{\bsfXi}{0}{bsfletters}{'004}
\DeclareMathSymbol{\ssfXi}{0}{ssfletters}{'004}
\DeclareMathSymbol{\bsfPi}{0}{bsfletters}{'005}
\DeclareMathSymbol{\ssfPi}{0}{ssfletters}{'005}
\DeclareMathSymbol{\bsfSigma}{0}{bsfletters}{'006}
\DeclareMathSymbol{\ssfSigma}{0}{ssfletters}{'006}
\DeclareMathSymbol{\bsfUpsilon}{0}{bsfletters}{'007}
\DeclareMathSymbol{\ssfUpsilon}{0}{ssfletters}{'007}
\DeclareMathSymbol{\bsfPhi}{0}{bsfletters}{'010}
\DeclareMathSymbol{\ssfPhi}{0}{ssfletters}{'010}
\DeclareMathSymbol{\bsfPsi}{0}{bsfletters}{'011}
\DeclareMathSymbol{\ssfPsi}{0}{ssfletters}{'011}
\DeclareMathSymbol{\bsfOmega}{0}{bsfletters}{'012}
\DeclareMathSymbol{\ssfOmega}{0}{ssfletters}{'012}

\newcommand{\fxfm}{\stackrel{\mathcal{F}}{\longleftrightarrow}}
\newcommand{\lxfm}{\stackrel{\mathcal{L}}{\longleftrightarrow}}
\newcommand{\zxfm}{\stackrel{\mathcal{Z}}{\longleftrightarrow}}

\DeclareMathOperator*{\gltop}{\gtreqless}
\newcommand{\glt}{\;\gltop^{\Hh=\svH_1}_{\Hh=\svH_0}\;}
\newcommand{\glty}{\;\gltop^{\Hh(\svy)=\svH_1}_{\Hh(\svy)=\svH_0}\;}
\newcommand{\gltby}{\;\gltop^{\Hh(\svby)=\svH_1}_{\Hh(\svby)=\svH_0}\;}
\DeclareMathOperator*{\geltop}{\genfrac{}{}{0pt}{}{\ge}{<}}
\newcommand{\gelty}{\;\geltop^{\Hh(\svy)=\svH_1}_{\Hh(\svy)=\svH_0}\;}
\newcommand{\geltby}{\;\geltop^{\Hh(\svby)=\svH_1}_{\Hh(\svby)=\svH_0}\;}
\renewcommand{\pe}{\Pr(e)}
\renewcommand{\defeq}{\triangleq}
\newcommand{\like}{\svlike}
\newcommand{\rvlike}{\mathssf{L}}
\newcommand{\sst}{\cl}
\newcommand{\svlike}{L}
\newcommand{\llike}{\rvllike}
\newcommand{\rvllike}{\cl}
\newcommand{\svllike}{l}
\newcommand{\bllike}{\rvbllike}
\newcommand{\rvbllike}{\boldsymbol{\cl}}
\newcommand{\svbllike}{\mathbf{l}}
\newcommand{\Qb}{\overline{Q}}
\renewcommand{\comb}[2]{\binom{#1}{#2}}


%% Random/sample variable/vector declarations.  Please add in alphabetical
%% order.  First section is for capitals.  Second for lower case.
% Capitals
\newcommand{\rvA}{{\mathssf{A}}} % A
\newcommand{\svA}{A}
\newcommand{\rvbA}{{\mathbsf{A}}}
\newcommand{\svbA}{{\mathbf{A}}}
\newcommand{\rvC}{{\mathssf{C}}} % A
\newcommand{\svC}{C}
\newcommand{\rvbC}{{\mathbsf{C}}}
\newcommand{\svbC}{{\mathbf{C}}}
\newcommand{\rvD}{{\mathssf{D}}} % D
\newcommand{\svD}{D}
\newcommand{\rvbD}{{\mathbsf{D}}}
\newcommand{\svbD}{{\mathbf{D}}}
\newcommand{\rvFh}{{\hat{\mathssf{F}}}}   % F
\newcommand{\rvF}{{\mathssf{F}}}
\newcommand{\rvHh}{{\hat{\mathssf{H}}}}   % H
\newcommand{\rvH}{{\mathssf{H}}}
\newcommand{\svH}{H}
\newcommand{\rvI}{{\mathssf{I}}}        % I
\newcommand{\svHh}{{\hat{\svH}}}
\newcommand{\rvL}{{\mathssf{L}}} % L
\newcommand{\svL}{L}
\newcommand{\rvN}{{\mathssf{N}}} % N
\newcommand{\rvP}{{\mathssf{P}}} % P
\newcommand{\rvR}{{\mathssf{R}}} % R
\newcommand{\rvRh}{{\hat{\rvR}}}
\newcommand{\rvS}{{\mathssf{S}}} % S
\newcommand{\rvSh}{{\hat{\rvS}}}
\newcommand{\rvT}{{\mathssf{T}}} % T 
\newcommand{\rvU}{{\mathssf{U}}} % U
\newcommand{\rvW}{{\mathssf{W}}} % W
\newcommand{\rvX}{{\mathssf{X}}}    % X, random variable
\newcommand{\svX}{X}
\newcommand{\rvXt}{{\tilde{\rvX}}}
\newcommand{\rvY}{{\mathssf{Y}}} % Y
\newcommand{\rvZ}{{\mathssf{Z}}} % Z

\newcommand{\rva}{{\mathssf{a}}} % a
\newcommand{\rvah}{{\hat{\rva}}}
\newcommand{\sva}{a}
\newcommand{\svah}{{\hat{\sva}}}
\newcommand{\rvba}{{\mathbsf{a}}}
\newcommand{\svba}{{\mathbf{a}}}
\newcommand{\rvb}{{\mathssf{b}}} % b
\newcommand{\rvc}{{\mathssf{c}}} % c
\newcommand{\rvch}{{\hat{\rvc}}}
\newcommand{\svc}{c}
\newcommand{\svch}{{\hat{\svc}}}
\newcommand{\rvbc}{{\mathbsf{c}}}
\newcommand{\svbc}{{\mathbf{c}}}

\newcommand{\rvd}{{\mathssf{d}}} % d
\newcommand{\rvdh}{{\hat{\rvd}}}
\newcommand{\svd}{d}
\newcommand{\svdh}{{\hat{\svd}}}
\newcommand{\rvbd}{{\mathbsf{d}}}
\newcommand{\svbd}{{\mathbf{d}}}



\newcommand{\rve}{{\mathssf{e}}} % e
\newcommand{\sve}{e}
\newcommand{\rvbe}{{\mathbsf{e}}}
\newcommand{\svbe}{{\mathbf{e}}}
\newcommand{\rvf}{{\mathssf{f}}} % f
\newcommand{\svf}{f}
\newcommand{\rvbf}{{\mathbsf{f}}}
\newcommand{\svbf}{{\mathbf{f}}}
\newcommand{\rvg}{{\mathssf{g}}} % g
\newcommand{\svg}{g}
\newcommand{\rvbg}{{\mathbsf{g}}}
\newcommand{\svbg}{{\mathbf{g}}}
\newcommand{\rvh}{{\mathssf{h}}} % h
\newcommand{\svh}{h}
\newcommand{\rvbh}{{\mathbsf{h}}}
\newcommand{\svbh}{{\mathbf{h}}}
\newcommand{\rvk}{{\mathssf{k}}} % k
\newcommand{\svk}{k}
\newcommand{\rvm}{{\mathssf{m}}} % m
\newcommand{\svm}{m}
\newcommand{\rvbm}{{\mathbsf{m}}}
\newcommand{\svbm}{{\mathbf{m}}}
\newcommand{\rvn}{{\mathssf{n}}} % n
\newcommand{\svn}{n}
\newcommand{\rvbn}{{\mathbsf{n}}}
\newcommand{\svbn}{{\mathbf{n}}}
\newcommand{\rvp}{{\mathssf{p}}} % p
\newcommand{\svp}{p}
\newcommand{\rvq}{{\mathssf{q}}} % q
\newcommand{\svq}{q}
\newcommand{\rvr}{{\mathssf{r}}} % r
\newcommand{\rvbr}{{\mathbsf{r}}}
\newcommand{\svr}{r}
\newcommand{\rvs}{{\mathssf{s}}} % s
\newcommand{\rvbs}{{\mathbsf{s}}}
\newcommand{\svs}{s}
\newcommand{\svbs}{{\mathbf{s}}}
\newcommand{\rvt}{{\mathssf{t}}} % t
\newcommand{\rvbt}{{\mathbsf{t}}}
\newcommand{\svt}{t}
\newcommand{\svbt}{{\mathbf{t}}}
\newcommand{\rvu}{{\mathssf{u}}} % u
\newcommand{\svu}{u}
\newcommand{\svuh}{{\hat{\svu}}}
\newcommand{\rvbu}{{\mathbsf{u}}}
\newcommand{\svbu}{{\mathbf{u}}}
\newcommand{\rvv}{{\mathssf{v}}} % v
\newcommand{\svv}{v}
\newcommand{\svvh}{{\hat{\svv}}}
\newcommand{\rvbv}{{\mathbsf{v}}}
\newcommand{\svbv}{{\mathbf{v}}}
\newcommand{\rvvh}{{\hat{\rvv}}}
\newcommand{\rvw}{{\mathssf{w}}} % w
\newcommand{\svw}{w}
\newcommand{\rvwh}{{\hat{\rvw}}}
\newcommand{\svwh}{{\hat{\svw}}}
\newcommand{\rvbw}{{\mathbsf{w}}}
\newcommand{\svbw}{{\mathbf{w}}}
\newcommand{\rvx}{{\mathssf{x}}} % x, random variable
\newcommand{\rvxh}{{\hat{\rvx}}}
\newcommand{\rvxt}{{\tilde{\rvx}}}
\newcommand{\svx}{x}       % sample value
\newcommand{\svxh}{{\hat{\svx}}}
\newcommand{\svxt}{{\tilde{\svx}}}
\newcommand{\rvbx}{{\mathbsf{x}}}
\newcommand{\rvbxh}{{\hat{\rvbx}}}
\newcommand{\rvbxt}{{\tilde{\rvbx}}}
\newcommand{\svbx}{{\mathbf{\svx}}}
\newcommand{\svbxt}{{\tilde{\svbx}}}
\newcommand{\svbxh}{{\hat{\mathbf{x}}}}
\newcommand{\rvy}{{\mathssf{y}}} % y
\newcommand{\rvyh}{{\hat{\mathssf{y}}}}
\newcommand{\svy}{y}
\newcommand{\rvyt}{{\tilde{\rvy}}}
\newcommand{\svyt}{{\tilde{\svy}}}
\newcommand{\svyh}{{\hat{\svy}}}
\newcommand{\rvby}{{\mathbsf{y}}}
\newcommand{\rvbyt}{{\tilde{\rvby}}}
\newcommand{\svby}{{\mathbf{y}}}
\newcommand{\svbyt}{{\tilde{\svby}}}
\newcommand{\rvz}{{\mathssf{z}}} % z
\newcommand{\rvzh}{{\hat{\rvz}}}
\newcommand{\rvzt}{{\tilde{\rvz}}}
\newcommand{\svz}{z}
\newcommand{\svzh}{{\hat{\svz}}}
\newcommand{\rvbz}{{\mathbsf{z}}}
\newcommand{\svbz}{{\mathbf{z}}}

% Handle uppercase Greek differently
\newcommand{\rvTh}{\ssfTheta}
\newcommand{\svTh}{\Theta}
\newcommand{\rvbTh}{\bsfTheta}
\newcommand{\svbTh}{\boldsymbol{\Theta}}
\newcommand{\rvPh}{\ssfPhi}
\newcommand{\svPh}{\Phi}
\newcommand{\rvbPh}{\bsfPhi}
\newcommand{\svbPh}{\boldsymbol{\Phi}}

\newcommand{\ddx}{\frac{\p}{\p \svx}}
\newcommand{\ddbx}{\frac{\p}{\p\svbx}}

%  --add new macros below this line--


==> styles/gww_chars.tex <==
% ABBREVIATIONS FOR CHARACTERS IN VARIOUS FONTS

% STANDARD CHARACTERS

\newcommand{\ba}{{\mathbf{a}}}
\newcommand{\bah}{{\hat{\ba}}}
\newcommand{\ah}{{\hat{a}}}
\newcommand{\Ah}{{\hat{A}}}
\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\at}{{\tilde{a}}}
\newcommand{\bat}{{\tilde{\ba}}}
\newcommand{\At}{{\tilde{A}}}
\newcommand{\bA}{{\mathbf{A}}}
\newcommand{\ac}{a^{\ast}}

\newcommand{\bb}{{\mathbf{b}}}
\newcommand{\bbt}{{\tilde{\bb}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\tb}{{\tilde{b}}}
\newcommand{\tB}{{\tilde{B}}}
\newcommand{\hb}{{\hat{b}}}
\newcommand{\hB}{{\hat{B}}}
\newcommand{\bB}{{\mathbf{B}}}

\newcommand{\bc}{{\mathbf{c}}}
\newcommand{\bch}{{\hat{\mathbf{c}}}}
\newcommand{\bC}{{\mathbf{C}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\ct}{{\tilde{c}}}
\newcommand{\Ct}{{\tilde{C}}}
\newcommand{\ctc}{\ct^{\ast}}

\newcommand{\bd}{{\mathbf{d}}}
\newcommand{\bD}{{\mathbf{D}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\hd}{{\hat{d}}}  % old: \dh
\newcommand{\dt}{{\tilde{d}}}
\newcommand{\bdt}{{\tilde{\bd}}}
\newcommand{\Dt}{{\tilde{D}}}
\newcommand{\dtc}{\dt^{\ast}}

\newcommand{\et}{{\tilde{e}}}
\newcommand{\bfe}{{\mathbf{e}}}
\newcommand{\bE}{{\mathbf{E}}}
\newcommand{\cE}{{\mathcal{E}}}
\newcommand{\cEt}{{\tilde{\cE}}}
\newcommand{\cEb}{{\bar{\cE}}}
\newcommand{\bcE}{{\mathbf{\cE}}}  % bf cal E doesn't exist

\newcommand{\bff}{{{\mathbf{f}}}}
\newcommand{\bF}{{\mathbf{F}}}
\newcommand{\cF}{{\mathcal{F}}}
\newcommand{\ft}{{\tilde{f}}}
\newcommand{\Ft}{{\tilde{F}}}
\newcommand{\Fh}{{\hat{F}}}
\newcommand{\ftc}{\ft^{\ast}}
\newcommand{\bft}{{\tilde{\bff}}}
\newcommand{\bFt}{{\tilde{\bF}}}
\newcommand{\fh}{{\hat{f}}}

\newcommand{\bg}{{\mathbf{g}}}
\newcommand{\gt}{{\tilde{g}}}
\newcommand{\bgt}{{\tilde{\bg}}}
\newcommand{\bG}{{\mathbf{G}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\Gt}{{\tilde{\bG}}}

\newcommand{\hti}{{\tilde{h}}}
\newcommand{\Hti}{{\tilde{H}}}
\newcommand{\bh}{{\mathbf{h}}}
\newcommand{\bht}{{\tilde{\bh}}}
\newcommand{\Hh}{{\hat{H}}}
\newcommand{\bH}{{\mathbf{H}}}
\newcommand{\bHh}{{\hat{\mathbf{H}}}}
\newcommand{\cH}{{\mathcal{H}}}

\newcommand{\ih}{{\hat{\imath}}}
\newcommand{\bI}{{\mathbf{I}}}
\newcommand{\cI}{{\mathcal{I}}}

\newcommand{\jh}{{\hat{\jmath}}}
\newcommand{\bJ}{{\mathbf{J}}}
\newcommand{\cJ}{{\mathcal{J}}}
\newcommand{\Jt}{{\tilde{J}}}

\newcommand{\bk}{{\mathbf{k}}}
\newcommand{\bK}{{\mathbf{K}}}
\newcommand{\Kt}{{\tilde{K}}}
\newcommand{\Kh}{{\hat{K}}}
\newcommand{\cK}{{\mathcal{K}}}

\newcommand{\cl}{\ell}
\newcommand{\bL}{{\mathbf{L}}}
\newcommand{\cL}{{\mathcal{L}}}

\newcommand{\mb}{{\mathbf{m}}}
\newcommand{\mh}{{\hat{m}}}
\newcommand{\bM}{{\mathbf{M}}}
\newcommand{\cM}{{\mathcal{M}}}


\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\Nt}{{\tilde{N}}}
\newcommand{\tN}{{\tilde{N}}}  % backward compatibility

\newcommand{\bo}{{\mathbf{o}}}
\newcommand{\cO}{{\mathcal{O}}}

\newcommand{\bp}{{\mathbf{p}}}
\newcommand{\bP}{{\mathbf{P}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\ph}{{\hat{p}}}
\newcommand{\Ph}{{\hat{P}}}

\newcommand{\bq}{{\mathbf{q}}}
\newcommand{\cQ}{{\mathcal{Q}}}
\newcommand{\bQ}{{\mathbf{Q}}}

\newcommand{\br}{{\mathbf{r}}}
\newcommand{\bR}{{\mathbf{R}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\Rt}{{\tilde{R}}}

\newcommand{\sh}{{\hat{s}}}
\newcommand{\sck}{{\check{s}}}
\newcommand{\shh}{{\Hat{\Hat{s}}}}
\newcommand{\bs}{{\mathbf{s}}}
\newcommand{\bsh}{{\hat{\mathbf{s}}}}
\newcommand{\bsc}{{\check{\mathbf{s}}}}
\newcommand{\bshh}{{\Hat{\Hat{\mathbf{s}}}}}
\newcommand{\bS}{{\mathbf{S}}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\st}{{\tilde{s}}}

\newcommand{\bT}{{\mathbf{T}}}
\newcommand{\cT}{{\mathcal{T}}}

\newcommand{\bu}{{\mathbf{u}}}
\newcommand{\bU}{{\mathbf{U}}}
\newcommand{\bUt}{{\tilde{\bU}}}
\newcommand{\ut}{{\tilde{u}}}
\newcommand{\cU}{{\mathcal{U}}}

\newcommand{\vh}{{\hat{v}}}
\newcommand{\bv}{{\mathbf{v}}}
\newcommand{\bV}{{\mathbf{V}}}
\newcommand{\cV}{{\mathcal{V}}}

\newcommand{\bw}{{\mathbf{w}}}
\newcommand{\bW}{{\mathbf{W}}}
\newcommand{\cW}{{\mathcal{W}}}

\newcommand{\bx}{{\mathbf{x}}}
\newcommand{\bxt}{{\tilde{\bx}}}
\newcommand{\xt}{{\tilde{x}}}
\newcommand{\Xt}{{\tilde{X}}}
\newcommand{\bX}{{\mathbf{X}}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\bXt}{{\tilde{\bX}}}
\newcommand{\xh}{{\hat{x}}}
\newcommand{\xc}{{\check{x}}}
\newcommand{\xhh}{{\Hat{\Hat{x}}}}
\newcommand{\bxh}{{\hat{\bx}}}
\newcommand{\bxc}{{\check{\bx}}}
\newcommand{\bxhh}{{\Hat{\hat{\bx}}}}

\newcommand{\cY}{{\mathcal{Y}}}
\newcommand{\by}{{\mathbf{y}}}
\newcommand{\byt}{{\tilde{\by}}}
\newcommand{\bY}{{\mathbf{Y}}}
\newcommand{\Yt}{{\tilde{Y}}}
\newcommand{\yt}{{\tilde{y}}}
\newcommand{\yh}{{\hat{y}}}

\newcommand{\zt}{{\tilde{z}}}
\newcommand{\zh}{{\hat{z}}}
\newcommand{\bz}{{\mathbf{z}}}
\newcommand{\bZ}{{\mathbf{Z}}}
\newcommand{\cZ}{{\mathcal{Z}}}

% GREEK CHARACTERS

\newcommand{\al}{\alpha}
\newcommand{\bal}{{\boldsymbol{\al}}}
\newcommand{\balh}{{\hat{\boldsymbol{\al}}}}
\newcommand{\alh}{{\hat{\al}}}

\newcommand{\bt}{\beta}
\newcommand{\btt}{{\tilde{\bt}}}
\newcommand{\btht}{{\hat{\bt}}}

\newcommand{\g}{\gamma}
\newcommand{\G}{\Gamma}
\newcommand{\bGa}{{\boldsymbol{\Gamma}}}
\newcommand{\gh}{{\hat{\g}}}

\newcommand{\de}{\delta}
\newcommand{\De}{\Delta}
\newcommand{\Deh}{{\hat{\Delta}}}
\newcommand{\bde}{{\boldsymbol{\de}}}
\newcommand{\bDe}{{\boldsymbol{\De}}}

\newcommand{\e}{\epsilon}
\newcommand{\eps}{\varepsilon}

\newcommand{\etah}{{\hat{\eta}}}
\newcommand{\bpi}{{\boldsymbol{\pi}}}

\newcommand{\pht}{{\tilde{\phi}}}
\newcommand{\Pht}{{\tilde{\Phi}}}

\newcommand{\pst}{{\tilde{\psi}}}
\newcommand{\Pst}{{\tilde{\Psi}}}

\newcommand{\s}{\sigma}
\newcommand{\sih}{\hat{\sigma}}

\newcommand{\z}{\zeta}
\newcommand{\ztt}{{\tilde{\z}}}
\newcommand{\ztb}{{\bar{\z}}}

% \newcommand{\th}{\theta} % symbol name used by other latex package
\newcommand{\thh}{{\hat{\theta}}}
\newcommand{\Thh}{{\hat{\Theta}}}
\newcommand{\Th}{\Theta}
\newcommand{\bth}{{\boldsymbol{\theta}}}
\newcommand{\bTh}{{\boldsymbol{\Theta}}}
\newcommand{\bThh}{{\hat{\bTh}}}
\newcommand{\Tht}{{\tilde{\Theta}}}

\newcommand{\la}{\lambda}
%\newcommand{\La}{\Lambda}
\newcommand{\lam}{\lambda}  % backward compatibility
\newcommand{\Lam}{\Lambda}  % backward compatibility
\newcommand{\bLa}{{\boldsymbol{\La}}}
\newcommand{\lah}{{\hat{\lam}}}

\newcommand{\bmu}{{\boldsymbol{\mu}}}

\newcommand{\bXi}{{\boldsymbol{\Xi}}}

\newcommand{\bPi}{{\boldsymbol{\Pi}}}

\newcommand{\rht}{{\tilde{\rho}}}
\newcommand{\rhc}{{\check{\rho}}}

\newcommand{\bSi}{{\boldsymbol{\Sigma}}}

\newcommand{\ups}{\upsilon}
\newcommand{\Ups}{\Upsilon}
\newcommand{\bUp}{{\boldsymbol{\Ups}}}

\newcommand{\bPs}{{\boldsymbol{\Psi}}}

\newcommand{\w}{\omega}
\newcommand{\wh}{{\hat{\omega}}}
\newcommand{\W}{\Omega}






==> styles/gww_defs.tex <==
% GWW DEFINITIONS AND ABBREVIATIONS

% TeX Defs

\usepackage[tbtags]{amsmath} % defines many math commands and
                 % subequations environment, etc
\usepackage{amssymb}  % get, among others, blackboard bold fonts
                      % defines extra symbols like \gtreqless, etc
\usepackage{verbatim} % get comment environment, + new verbatim
% \usepackage{amsxtra}  % get, eg, \accentedsymbol

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argsup}{arg\,sup}
\DeclareMathOperator*{\arginf}{arg\,inf}
\DeclareMathOperator{\erfc}{erfc}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\cum}{cum}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\adj}{adj}
\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator*{\lms}{l.i.m.\,}
\newcommand{\varop}[1]{\var\left[{#1}\right]}
\newcommand{\covop}[2]{\cov\left({#1},{#2}\right)}

\newcommand{\p}{\partial}

% LIST ENVIRONMENTS

\newcounter{actr}
\newenvironment{alist}%
{\begin{list}{(\alph{actr})}{\usecounter{actr}}}{\end{list}}

\newcounter{ictr}
\newenvironment{ilist}%
{\begin{list}{(\roman{ictr})}{\usecounter{ictr}}}{\end{list}}

\iffalse

% SPACING ENVIRONMENTS

\newenvironment{singlespace}%
{\begin{spacing}{1}}{\end{spacing}}

\newenvironment{onehalfspace}% for 11pt font
{\begin{spacing}{1.21}}{\end{spacing}}

\newenvironment{doublespace}% for 11pt font
{\begin{spacing}{1.62}}{\end{spacing}}

\fi

% THEOREM ENVIRONMENTS

% \newtheorem{thm}{Theorem}
% \newtheorem{lemma}{Lemma}
% \newtheorem{claim}{Claim}
% \newtheorem{corol}{Corollary}
% \newtheorem{prop}{Proposition}
% \newtheorem{conj}{Conjecture}
% \newtheorem{defn}{Definition}
%\newenvironment{proof}%
%{\noindent{\em Proof: } \begin{singlespace} \small \noindent}%
%{\noindent\qed \end{singlespace}}
%\newenvironment{new-proof}[1]%
%{{\em Proof of #1: } \begin{singlespace} \small \noindent}%
%{\ \noindent\qed \end{singlespace}}

\iffalse
\newenvironment{proof}%
{\noindent{\em Proof: } \small \noindent}%
{\noindent\qed }
\newenvironment{new-proof}[1]%
{{\em Proof of #1: } \small \noindent}%
{\ \noindent\qed }
\fi
\newcommand{\abs}[1]{\left|#1\right|}
%\newcommand{\comb}[2]{{#1\choose#2}}
\newcommand{\comb}[2]{\binom{#1}{#2}}
\newcommand{\ie}{i.e.}
\newcommand{\eg}{e.g.}
\newcommand{\etc}{etc.}
\newcommand{\viz}{viz.}
\newcommand{\etal}{et al.}
\newcommand{\cf}{cf.}

\newcommand{\vect}[3]{\begin{bmatrix} #1 & #2 & \cdots & #3 \end{bmatrix}^\T}

\newcommand{\dsp}{.5\baselineskip}             % double space amount
\newcommand{\down}{\vspace{\dsp}}              % double space command
\newcommand{\ddown}{\vspace{\baselineskip}}    % quadruple space command
\newcommand{\spec}{\hspace*{1pt}}              % little bit of space
\newcommand{\ds}{\displaystyle}                % abbreviation
\newcommand{\ts}{\textstyle}                % abbreviation
\newcommand{\nin}{\noindent}                   % noindent abbreviation
\newcommand{\cvar}[1]{\mathrm{var_{#1}\,}}
\newcommand{\qed}{\rule[0.1ex]{1.4ex}{1.6ex}}
\newcommand{\mycap}[2]{\caption{\sl #2 \label{#1}}}
\newcommand{\subcap}[1]{{\begin{center}\sl #1\end{center}}}
\newcommand{\ditem}[1]{\item[#1 \hspace*{\fill}]}
\newcommand{\appfig}{\vspace*{1in}\begin{center} Figure appended to
                       end of manuscript. \end{center} \vspace*{1in}}
\newcommand{\psx}[1]{\centerline{\epsfxsize=6in \epsfbox{#1}}}
\newcommand{\psy}[1]{\centerline{\epsfysize=7in \epsfbox{#1}}}
\newcommand{\psxs}[2]{\centerline{\epsfxsize=#1in \epsfbox{#2}}}
\newcommand{\psxsbb}[3]{\centerline{\epsfxsize=#1in \epsfbox[#3]{#2}}}
\newcommand{\psys}[2]{\centerline{\epsfysize=#1in \epsfbox{#2}}}
\newcommand{\convsamp}[3]{\left.\left\{#1 \ast #2\right\}\right|_{#3}}
\newcommand{\gap}{\qquad}
\newcommand{\order}[1]{\mathcal{O}\left(#1\right)}
\newcommand{\arror}[3]{\begin{cases} #1 & #2 \\
                                     #3 & \text{otherwise} \end{cases}}
\newcommand{\arrorc}[3]{\begin{cases} #1 & #2 \\
                                     #3 & \text{otherwise,} \end{cases}}
\newcommand{\arrorp}[3]{\begin{cases} #1 & #2 \\
                                     #3 & \text{otherwise.} \end{cases}}
\newcommand{\darror}[4]{\begin{cases} #1 & #2 \\ #3 & #4 \end{cases}}
% \newcommand{\defeq}{\stackrel{\triangle}{=}}
\newcommand{\defeq}{\stackrel{\Delta}{=}}
\newcommand{\msconv}{\stackrel{\mathrm{m.s.}}{\longrightarrow}}
\newcommand{\pwaeconv}{\stackrel{\mathrm{p.w.a.e.}}{\longrightarrow}}
\newcommand{\peq}{\stackrel{\mathcal{P}}{=}}
% \newcommand{\glt}{ \begin{array}{c} \Hh=H_1 \\
%  \renewcommand{\arraystretch}{.3}
%  \begin{array}{c} > \\ < \end{array}
%  \renewcommand{\arraystretch}{1} \\ \Hh=H_0 \end{array}}

\hyphenation{or-tho-nor-mal}
\hyphenation{wave-let wave-lets}

\newcommand{\crb}{Cram\'{e}r-Rao}  % obsolete
\newcommand{\CR}{Cram\'{e}r-Rao}
\newcommand{\KL}{Karhunen-Lo\`{e}ve}
\newcommand{\sE}{\sqrt{E_0}}
\newcommand{\pe}{\Pr(\eps)}
\newcommand{\jw}{j\w}
\newcommand{\ejw}{e^{j\w}}
\newcommand{\ejv}{e^{j\nu}}
\newcommand{\wo}{{\w_0}}
\newcommand{\woh}{{\wh_0}}
\newcommand{\sumi}[1]{\sum_{#1=-\infty}^{+\infty}}
\newcommand{\inti}{\int_{-\infty}^{+\infty}}
\newcommand{\intp}{\int_{-\pi}^{\pi}}
\newcommand{\nintp}{\frac{1}{2\pi}\int_{-\pi}^{\pi}}
\newcommand{\inth}{\int_{0}^{\infty}}
\newcommand{\E}[1]{E\left[{#1}\right]}
\newcommand{\bigE}[1]{E\bigl[{#1}\bigr]}
\newcommand{\BigE}[1]{E\Bigl[{#1}\Bigr]}
\newcommand{\biggE}[1]{E\biggl[{#1}\biggr]}
\newcommand{\BiggE}[1]{E\Biggl[{#1}\Biggr]}
\newcommand{\Prob}[1]{\Pr\left[{#1}\right]}
\newcommand{\Pu}[1]{\Pr\left[{#1}\right]} % obsolete; same as \Prob now
\newcommand{\Pc}[2]{\Pr\left[{#1}\mid{#2}\right]}  % obsolete
\newcommand{\Pcb}[2]{\Pr\left[{#1}\Bigm|{#2}\right]} % obsolete
\newcommand{\Q}[1]{\mathcal{Q}\left({#1}\right)}
\newcommand{\FT}[1]{\mathcal{F}\left\{{#1}\right\}}
\newcommand{\LT}[1]{\mathcal{L}\left\{{#1}\right\}}
\newcommand{\ZT}[1]{\mathcal{Z}\left\{{#1}\right\}}
%\newcommand{\reals}{\mathbf{R}}
\newcommand{\reals}{\mathbb{R}}
%\newcommand{\ints}{\mathbf{Z}}
\newcommand{\ints}{\mathbb{Z}}
\newcommand{\compls}{\mathbb{C}}
\newcommand{\nats}{\mathbb{N}}
\newcommand{\rats}{\mathbb{Q}}
\newcommand{\ltwor}{L^2(\reals)}
\newcommand{\ltwoz}{\ell^2(\ints)}
\newcommand{\ltwow}{L^2(\Omega)}
% \newcommand{\ltwo}{\mathbf{L}^2}
% \newcommand{\ltwor}{\mathbf{L}^2 (\reals)}
% \newcommand{\ltwoz}{\mathbf{l}^2 (\ints)}
\newcommand{\sys}[1]{\mathcal{S}\left\{#1\right\}}
\newcommand{\nn}{\nonumber}

\newcommand{\ip}[2]{\left\langle{#1},{#2}\right\rangle}
\newcommand{\di}[2]{d\left({#1},{#2}\right)}
\newcommand{\ceil}[1]{\lceil{#1}\rceil}
\newcommand{\floor}[1]{\lfloor{#1}\rfloor}
\newcommand{\phase}{\measuredangle}

\newcommand{\Ht}{\mathrm{H}}
\newcommand{\T}{{\mathrm{T}}}
% \newcommand{\R}{\Re\mathit{e}}
% \newcommand{\I}{\Im\mathit{m}}
\DeclareMathOperator{\R}{Re}
\DeclareMathOperator{\I}{Im}


==> system_model.tex <==
\section{System Model}
\label{sec:sparse.system_model}

\subsection*{\normalsize \textsf{Sparsity of the main channel}}

Consider an orthogonal frequency-division multiplexing (OFDM) system with symbol duration $T$ and bandwidth $W$. Two users, Alice and Bob, transmit a sounding sequence $\bs = [s_1, s_2, \cdots, s_{K}]^T$, $K=\lceil TW \rceil$, to each other over a reciprocal frequency selective fading channel within a coherent time. Let $\taum$ be the maximum delay spread of the channel. The sequence input to the channel is $[\tilbs^T, \bs^T]^T$ with a cyclic prefix $\tilbs = [s_{K-\tilL+2}, \cdots, s_{K}]^T$ where $\tilL = \lceil \taum W \rceil$. The length-$K$ channel outputs at two users are
\begin{subequations}\label{equ:sparse_channel_output}
\begin{align}
    \bx &= \bS \bh + \bn_1 \\
    \text{and} \qquad
    \by &= \bS \bh + \bn_2 \ ,
\end{align}
\end{subequations}
respectively. Here $\bh = [h_1, h_2, \cdots, h_{\tilL}]^T$ is the sampled (virtual) channel coefficient vector \cite{sayeed_bookchapter}. $\bx = [x_1, x_2, \cdots, x_K]^T$ is length-$K$ channel outputs at Alice and $\by = [y_1, y_2, \cdots, y_K]^T$ is the output at Bob. $\bS$ is a $K$-by-$L$ Toeplitz matrix
\begin{equation*}
    \bS =
    \left[
    \begin{array}{cccc}
      \bs_{1}^T & \bs_{2}^T & \cdots & \bs_{\tilL}^T
    \end{array}
    \right]
    = \left(
      \begin{array}{ccccc}
        s_1 & s_K & s_{K-1} & \cdots & s_{K-\tilL+2} \\
        s_2 & s_1 & s_{K}  & \cdots & s_{K-\tilL+3} \\
        \vdots &  \vdots & \ddots &  & \vdots \\
        s_{K} & s_{K-1} &  & \cdots & s_{K-\tilL+1} \\
      \end{array}
    \right) \ ,
\end{equation*}
where $\bs_{\ell}$ is the right circular shift sequence of $\bs$ with step $\ell-1$.
It is known from literature that the optimal sounding sequence is a statistically white sequence (\eg, \cite{HaykinAFT}), thus we assume $\bS$ has orthogonal columns and $\bS^{H}\bS = P \bI_{L}$.
$\bn_1$ and $\bn_2$ are independent $\randcn{\mathbf{0}}{\nvar_a \bI_{K}}$ and $\randcn{\mathbf{0}}{\nvar_b \bI_{K}}$ noise vectors, respectively.
%
We assume the channel coefficient $h_\ell$ is independent $\randcn{0}{\nu^2_\ell}$ and with the total channel power is normalized to one, \ie, $\sum_{\ell=1}^L \nu^2_\ell = 1$.
The maximum number of resolvable paths is $L = \lceil \taum W \rceil$.

In a \emph{rich scattering environment}, there are a significant number of scattered paths in each of the resolvable delay bins, resulting non-vanishing variance $\nu^2_\ell$ for all $\ell \in [1:L]$. Thus $L$ is the  degrees-of-freedom (DoF) in the channel. Furthermore, the channel DoF  increases \emph{linearly} as increasing $W$. This leads to a parallel channel studied in Section \ref{sec:GEDMMS.parallel_channel}.
% **************
However, when the physical scattering is sparse, there are very few or no paths in some of the delay bins and such $h_\ell$ will be zero. We consider a model that the effective DoF in the channel follows the sub-linear law \cite{Raghavan05, Raghavan2011}:
\begin{equation}\label{equ:sublinear_law}
    L = (\taum W)^{\delta}, \qquad \delta \in (0,1) \ .
\end{equation}
The channel DoF is propositional to $W^\delta$  and we call the channel is \emph{$\delta$-sparse}.
A rich channel is equivalent to $\delta=1$. To simplify the problem, we assume in an $\delta$-sparse channel, the channel is still has expressions as in \eqref{equ:sparse_channel_output} while the dimension of $\bh$ and column dimension of $\bS$ is changed according to \eqref{equ:sublinear_law}.
% there are $\Leff$ out of $L$ elements in $\bh$ are non-zero, all the others are zero. Without loss of generality, we assume


\subsection*{\normalsize \textsf{Correlation to Eve's channel}}

To get meaningful observations, Eve is assumed to be located close to one of the users, say Bob. Her channel output is
\begin{equation}\label{equ:sparse_Eve_output}
    \bz = \bS \tilbh + \bn_3
\end{equation}
where the noise is $\randcn{\mathbf{0}}{\nvar_e \bI_{K}}$. The channel coefficient vector $\tilbh$ is also $\delta$-sparse while the non-zero elements in  $\tilbh$ may or may not overlap with those in $\bh$. We consider a simple statistical model \cite{chou_isit10} with parameters $(\theta, \eta)$ for the correlation between $\bh$ and $\tilbh$:
\begin{itemize}
  \item \emph{Correlation of non-zero pattern between $\bh$ and $\tilbh$}: We introduce independent $\randBern{\theta}$ auxiliary random variables $\bQ = [Q_1, \cdots, Q_L]$ such that for each $\ell\in[1:L]$
      \begin{equation}\label{equ:overlap_model}
         \tilh_\ell = Q_\ell \hath_\ell + (1-Q_\ell) \hath'_\ell \ .
      \end{equation}
      This means $\tilh_\ell$ can be represented by one of two variables ($\hath_\ell$ and $\hath'_\ell$) controlled by $Q_\ell$, where $\hath_\ell$ is correlated with $h_\ell$ but $\hath'_\ell$ is not as we define below.
      This $Q_\ell$ variable is used to model the effect that in a sparse environment, the paths in the main channel may or may not share a common overlap with those in Eve's channel.

  \item \emph{Correlation coefficients}:
      The correlation coefficient between $h_\ell$ and $\hath_\ell$ (and $\hath'_\ell$) is
      \begin{align*}
         &\rho(h_\ell, \hath_\ell) = \eta \ , \\
         &\rho(h_\ell, \hath'_\ell) = 0 \ .
      \end{align*}
\end{itemize}

To generate a secret key, the users  use the vector channel \eqref{equ:sparse_channel_output} (and \eqref{equ:sparse_Eve_output}) $n$ times, each with i.i.d. $\bh$ (and $\tilbh$), and follows the protocol described in Section \ref{sec:edms.system_setting}.




==> system_model2.tex <==
\section{System Model}
\label{sec:sparse.system_model}

\subsection*{\normalsize \textsf{Sparsity of the main channel}}

We consider a system using orthogonal frequency-division multiplexing (OFDM) signaling. 
Let $T$ denote the signal duration in time and let $W$ denote the signal bandwidth. The orthogonal Fourier basis in an OFDM system is
\begin{equation*}
    \phi_m(t) = 
    \left\{
        \begin{array}{cc}
          \frac{1}{\sqrt{T}} e^{j2\pi m W_0 t} & \text{if~} 0 \le t\le T \\
          0 & \text{else} 
        \end{array}
    \right.
\end{equation*}
where $W_0 = \frac{1}{T}$ and $m \in [0: M-1]$, $M = \lceil\frac{W}{W_0}\rceil = \lceil TW \rceil$. 
The transmitted signal can be represented as 
\begin{equation*}
    s(t) = \sum_{m=0}^{M-1} s_m \phi_m(t), \quad 0\le t \le T \ .
\end{equation*}
The received signal from a frequency selective channel is $r(t) = h(t) * s(t) + w(t)$.
When channel has maximum delay spread $\taum$, $h(t)$ is the channel impulse response and is modeled as
\begin{equation*}
    h(t) = \sum_{k=1}^{N_p} \beta_k \delta(t- \tau_k) .
\end{equation*}
where $N_p$ is the total number of propagation paths, each with delay $\tau_k \in [1,\taum]$ and gain $\beta_k$. Without loss of generality, we assume $\sum_{k=1}^{N_p} \rvE[|\beta_k|^2] = 1$. 
$w(t)$ is a complex zero-mean white Gaussian noise process with autocorrelation function $E[w(t_1)w^*(t_2)] = \nvar \delta(t_1 -t_2)$.

Projecting the received signal onto the Fourier basis to yield
\begin{align}\label{equ:ofdm_channel_output}
    x_m &= \langle r(t), \phi_m(t) \rangle  = \sum_j H_j s_j  \langle \phi_j(t), \phi_m(t) \rangle 
                + \langle w(t), \phi_m(t) \rangle = H_m s_m + w_m \ .
\end{align}
Noise $w_m$ is $\randcn{0}{\nvar}$. $H_m$ is the frequency domain channel coefficient 
\begin{equation} \label{equ:freq_channel_coeff}
    H_m  = \sum_{k=1}^{N_p} \beta_k e^{-2\pi m \tau_k W_0} 
        \thickapprox  \sum_{\ell=0}^{L_{max}-1} h_\ell e^{-j 2 \pi m \frac{\ell}{M}} \quad \text{where~}L_{max} = \lceil \taum W \rceil
\end{equation}
and with variance 
\begin{equation*}
    \nu_m^2 = \rvE[|H_m|^2] = \sum_{k=1}^{N_p} \rvE[|\beta_k|^2] = 1 
\end{equation*}
%
for $0 \le m < M$. The $\{h_\ell\}$ in \eqref{equ:freq_channel_coeff} are the sampled (virtual) channel coefficients \cite{sayeed_bookchapter}. The $\ell$-th sampled channel coefficient is approximated as a sum of $\beta_k$ for the paths in the resolvable (disjointed) delay bin $\calB_\ell = (\frac{\ell-0.5}{W}, \frac{\ell+0.5}{W}]$, \ie,
\begin{equation*}
    h_\ell \thickapprox  \sum_{k:\tau_k \in \calB_\ell} \beta_k \ .
\end{equation*}
Thus the coefficients $\{h_\ell\}$ are independent of each other. The number of non-zero $h_\ell$, denoted by $L$, captures the \emph{degrees-of-freedom} (DoF) in the channel.
The channel DoF is decided by the signal bandwidth $W$ (which determines the resolvable bin size) and the scattering environment (which determines $\{\tau_k\}$). 
In a \emph{rich scattering environment}, there are a significant number of scattered paths in each of the delay bins, so $L = L_{max}$ which increases \emph{linearly} with $W$.
%
However, when the physical scattering is sparse, there are very few or no paths in some of the delay bins so that such $h_\ell$ would be zero. We consider a model that the effective DoF in the channel follows the \emph{sub-linear} law \cite{Raghavan05, Raghavan2011}:
\begin{equation}\label{equ:sublinear_law}
    L = (\taum W)^{\delta}, \qquad \delta \in (0,1) \ .
\end{equation}
We call such a channel is \emph{$\delta$-sparse}.


The frequency channel coefficients $\{H_m\}$ in \eqref{equ:freq_channel_coeff} are not independent. In this work, we consider a \emph{block fading} channel in which there are $L$ coherence frequency bands. The channel coefficients in each coherence band are identical, \ie
\begin{equation*}
    [ \underbrace{H_1 \cdots H_1}_{\text{band~}1}, \underbrace{H_2 \cdots H_2}_{\text{band~}2}, \cdots, 
            \underbrace{H_L \cdots H_L}_{\text{band~}L} ]
\end{equation*}


Since the correlated source for secret key generation are from the channel randomness, we can simplify the channel outputs to a size-$L$ vector, one for each coherence band. The channel outputs at Alice and Bob are
\begin{subequations}\label{equ:sparse_channel_output}
\begin{align}
    \bx &= \bS \bh + \bw_1 \\
    \by &= \bS \bh + \bw_2
\end{align}
\end{subequations}
where $\bh$, and $\bx$, $\by$ and $\bw_j$ are $L \times 1$ vectors. $\bS = \diag([s_1, \cdots, s_L])$ represent the sounding symbols in each coherence band. 

*************************

Consider a system with signal bandwidth $W$. Two users, Alice and Bob, transmit a sounding sequence $\bs = [s_1, s_2, \cdots, s_{L+K-1}]^T$ to each other over a reciprocal frequency selective fading channel within a coherent time. The channel outputs are
\begin{subequations}\label{equ:sparse_channel_output}
\begin{align}
    \bx &= \bS \bh + \bw_1 \\
    \by &= \bS \bh + \bw_2
\end{align}
\end{subequations}
where $\bh = [h_1, h_2, \cdots, h_L]^T$ and $\bx = [x_1, x_2, \cdots, x_K]^T$ is $K$-length channel outputs and $\bS$ is a $K$-by-$L$ Toeplitz matrix
\begin{equation*}
    \bS =
    \left[
    \begin{array}{cccc}
      \bs_{L}^T & \cdots & \bs_{2}^T & \bs_{1}^T
    \end{array}
    \right]
    = \left(
      \begin{array}{ccccc}
        s_L & s_{L-1} & \cdots & s_2 & s_1 \\
        s_{L+1} & s_L & s_{L-1} & \cdots & s_2 \\
        \vdots &   & \ddots &  & \vdots \\
        s_{L+K-1} & s_{L+K-1} &  & \cdots & s_K \\
      \end{array}
    \right) \ ,
\end{equation*}
where $\bs_{\ell}$ is a length-$K$ subsequence of $\bs$ with starting index $\ell$.
It is known from literature that the optimal sounding sequence is a statistically white sequence (\eg, \cite{HaykinAFT}), thus we assume $\bS$ has orthogonal columns and $\bS^{H}\bS = P \bI_{L}$.
$\bn_1$ and $\bn_2$ are independent $\randcn{\mathbf{0}}{\nvar_a \bI_{K}}$ and $\randcn{\mathbf{0}}{\nvar_b \bI_{K}}$ noise vectors, respectively.
%
We assume the channel coefficient $h_\ell$ is independent $\randcn{0}{\nu^2_\ell}$ and with the total channel power is normalized to one, \ie, $\sum_{\ell=1}^L \nu^2_\ell = 1$.
The maximum number of resolvable paths is $L = \lceil \taum W \rceil$.


In a \emph{rich scattering environment}, there are a significant number of scattered paths in each of the resolvable delay bins, resulting non-vanishing variance $\nu^2_\ell$ for all $\ell \in [1:L]$. Thus $L$ is the  degrees-of-freedom (DoF) in the channel. Furthermore, the channel DoF  increases \emph{linearly} as increasing $W$. This leads to a parallel channel studied in Section \ref{sec:GEDMMS.parallel_channel}.
% **************
However, when the physical scattering is sparse, there are very few or no paths in some of the delay bins and such $h_\ell$ will be zero. We consider a model that the effective DoF in the channel follows the sub-linear law \cite{Raghavan05, Raghavan2011}:
\begin{equation}\label{equ:sublinear_law}
    L = (\taum W)^{\delta}, \qquad \delta \in (0,1) \ .
\end{equation}
The channel DoF is propositional to $W^\delta$  and we call the channel is \emph{$\delta$-sparse}.
A rich channel is equivalent to $\delta=1$. To simplify the problem, we assume in an $\delta$-sparse channel, the channel is still has expressions as in \eqref{equ:sparse_channel_output} while the dimension of $\bh$ and column dimension of $\bS$ is changed according to \eqref{equ:sublinear_law}.
% there are $\Leff$ out of $L$ elements in $\bh$ are non-zero, all the others are zero. Without loss of generality, we assume


\subsection*{\normalsize \textsf{Correlation to Eve's channel}}

To get meaningful observations, Eve is assumed to be located close to one of the users, say Bob. Her channel output is
\begin{equation}\label{equ:sparse_Eve_output}
    \bz = \bS \tilbh + \bn_3
\end{equation}
where the noise is $\randcn{\mathbf{0}}{\nvar_e \bI_{K}}$. The channel coefficient vector $\tilbh$ is also $\delta$-sparse while the non-zero elements in  $\tilbh$ may or may not overlap with those in $\bh$. We consider a simple statistical model \cite{chou_isit10} with parameters $(\theta, \eta)$ for the correlation between $\bh$ and $\tilbh$:
\begin{itemize}
  \item \emph{Correlation of non-zero pattern between $\bh$ and $\tilbh$}: We introduce independent $\randBern{\theta}$ auxiliary random variables $\bQ = [Q_1, \cdots, Q_L]$ such that for each $\ell\in[1:L]$
      \begin{equation}\label{equ:overlap_model}
         \tilh_\ell = Q_\ell \hath_\ell + (1-Q_\ell) \hath'_\ell \ .
      \end{equation}
      This means $\tilh_\ell$ can be represented by one of two variables ($\hath_\ell$ and $\hath'_\ell$) controlled by $Q_\ell$, where $\hath_\ell$ is correlated with $h_\ell$ but $\hath'_\ell$ is not as we define below.
      This $Q_\ell$ variable is used to model the effect that in a sparse environment, the paths in the main channel may or may not share a common overlap with those in Eve's channel.

  \item \emph{Correlation coefficients}:
      The correlation coefficient between $h_\ell$ and $\hath_\ell$ (and $\hath'_\ell$) is
      \begin{align*}
         &\rho(h_\ell, \hath_\ell) = \eta \ , \\
         &\rho(h_\ell, \hath'_\ell) = 0 \ .
      \end{align*}
\end{itemize}

To generate a secret key, the users  use the vector channel \eqref{equ:sparse_channel_output} (and \eqref{equ:sparse_Eve_output}) $n$ times, each with i.i.d. $\bh$ (and $\tilbh$), and follows the protocol described in Section \ref{sec:edms.system_setting}.



